A general model-checking procedure for semiparametric accelerated failure time models

We propose a set of goodness-of-fit tests for the semiparametric accelerated failure time (AFT) model, including an omnibus test, a link function test, and a functional form test. This set of tests is derived from a multi-parameter cumulative sum process shown to follow asymptotically a zero-mean Gaussian process. Its evaluation is based on the asymptotically equivalent perturbed version, which enables both graphical and numerical evaluations of the assumed AFT model. Empirical p-values are obtained using the Kolmogorov-type supremum test, which provides a reliable approach for estimating the significance of both proposed un-standardized and standardized test statistics. The proposed procedure is illustrated using the induced smoothed rank-based estimator but is directly applicable to other popular estimators such as non-smooth rank-based estimator or least-squares estimator.Our proposed methods are rigorously evaluated using extensive simulation experiments that demonstrate their effectiveness in maintaining a Type I error rate and detecting departures from the assumed AFT model in practical sample sizes and censoring rates. Furthermore, the proposed approach is applied to the analysis of the Primary Biliary Cirrhosis data, a widely studied dataset in survival analysis, providing further evidence of the practical usefulness of the proposed methods in real-world scenarios. To make the proposed methods more accessible to researchers, we have implemented them in the R package afttest, which is publicly available on the Comprehensive R Archieve Network.

==> code/figure_pbc01_mis_unstd.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_omni_mis_unstd.eps} \\
	    \caption{afttestplot: pbc unstandardized omni function test} \label{fig:pbc01_omni_mis_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_link_mis_unstd.eps} \\
	    \caption{afttestplot: unstandardized link function test} \label{fig:pbc01_link_mis_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form1_mis_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc01_form1_mis_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form2_mis_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc01_form2_mis_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form3_mis_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc01_form3_mis_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form4_mis_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc01_form4_mis_unstd} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:pbc01:mis:unstd} Three simple graphs}
\end{figure}

==> code/figure_pbc01_mns_std.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_omni_mns_std.eps} \\
	    \caption{afttestplot: pbc standardized omni function test} \label{fig:pbc01_omni_mns_std} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_link_mns_std.eps} \\
	    \caption{afttestplot: standardized link function test} \label{fig:pbc01_link_mns_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form1_mns_std.eps} \\
	    \caption{afttestplot: standardized form function test} \label{fig:pbc01_form1_mns_std} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form2_mns_std.eps} \\
	    \caption{afttestplot: standardized form function test} \label{fig:pbc01_form2_mns_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form3_mns_std.eps} \\
	    \caption{afttestplot: standardized form function test} \label{fig:pbc01_form3_mns_std} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form4_mns_std.eps} \\
	    \caption{afttestplot: standardized form function test} \label{fig:pbc01_form4_mns_std} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:pbc01:mns:std} Three simple graphs}
\end{figure}

==> code/figure_pbc01_mns_unstd.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_omni_mns_unstd.eps} \\
	    \caption{afttestplot: pbc unstandardized omni function test} \label{fig:pbc01_omni_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_link_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized link function test} \label{fig:pbc01_link_mns_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form1_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc01_form1_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form2_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc01_form2_mns_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form3_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc01_form3_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc01_form4_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc01_form4_mns_unstd} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:pbc01:mns:unstd} Three simple graphs}
\end{figure}

==> code/figure_pbc02_mis_unstd.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_omni_mis_unstd.eps} \\
	    \caption{afttestplot: pbc unstandardized omni function test} \label{fig:pbc02_omni_mis_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_link_mis_unstd.eps} \\
	    \caption{afttestplot: unstandardized link function test} \label{fig:pbc02_link_mis_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form1_mis_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc02_form1_mis_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form2_mis_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc02_form2_mis_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form3_mis_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc02_form3_mis_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form4_mis_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc02_form4_mis_unstd} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:pbc01:mis:unstd} Three simple graphs}
\end{figure}

==> code/figure_pbc02_mns_std.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_omni_mns_std.eps} \\
	    \caption{afttestplot: pbc standardized omni function test} \label{fig:pbc02_omni_mns_std} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_link_mns_std.eps} \\
	    \caption{afttestplot: standardized link function test} \label{fig:pbc02_link_mns_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form1_mns_std.eps} \\
	    \caption{afttestplot: standardized form function test} \label{fig:pbc02_form1_mns_std} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form2_mns_std.eps} \\
	    \caption{afttestplot: standardized form function test} \label{fig:pbc02_form2_mns_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form3_mns_std.eps} \\
	    \caption{afttestplot: standardized form function test} \label{fig:pbc02_form3_mns_std} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form4_mns_std.eps} \\
	    \caption{afttestplot: standardized form function test} \label{fig:pbc02_form4_mns_std} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:pbc01:mns:std} Three simple graphs}
\end{figure}

==> code/figure_pbc02_mns_unstd.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_omni_mns_unstd.eps} \\
	    \caption{afttestplot: pbc unstandardized omni function test} \label{fig:pbc02_omni_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_link_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized link function test} \label{fig:pbc02_link_mns_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form1_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc02_form1_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form2_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc02_form2_mns_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form3_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc02_form3_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/pbc02_form4_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test} \label{fig:pbc02_form4_mns_unstd} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:pbc01:mns:unstd} Three simple graphs}
\end{figure}

==> code/figure_sim1_mis_std.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_omni_mis_std.eps} \\
	   % \caption{afttestplot: standardized omni function test with \texttt{mis} for model \eqref{model:sim1}} \label{fig:sim1_omni_mis_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_link_mis_std.eps} \\
	   % \caption{afttestplot: standardized link function test with \texttt{mis} for model \eqref{model:sim1}} \label{fig:sim1_link_mis_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_form_mis_std.eps} \\
	   % \caption{afttestplot: standardized form function test with \texttt{mis} for model \eqref{model:sim1}} \label{fig:sim1_form_mis_std} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:sim1:mis:std} Plots of sample paths based on the proposed standardized test procedures for Simulation scenario 1 with $\gamma = 0.3$, 20\% censoring rate and the sample size of 300. $x$-axis indicates the rank of the log transformed residuals. The sample path for the test statistic (red) overlays by 50 approximated sample paths under the null (grey) are displayed. Top panel is the plot for the omnibus test under the different quantiles of covariates. Bottom two panels are the plots for testing the link function (left) and functional form (right)}
\end{figure}

==> code/figure_sim1_mis_unstd.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_omni_mis_unstd.eps} \\
	   % \caption{afttestplot: unstandardized omni function test with \texttt{mis} for model \eqref{model:sim1}} \label{fig:sim1_omni_mis_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_link_mis_unstd.eps} \\
	   % \caption{afttestplot: unstandardized link function test with \texttt{mis} for model \eqref{model:sim1}} \label{fig:sim1_link_mis_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_form_mis_unstd.eps} \\
	   % \caption{afttestplot: unstandardized form function test with \texttt{mis} for model \eqref{model:sim1}} \label{fig:sim1_form_mis_unstd} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:sim1:mis:unstd} Plots of sample paths based on the proposed un-standardized test procedures for Simulation scenario 1 with $\gamma = 0.3$, 20\% censoring rate and the sample size of $300$. $x$-axis indicates the rank of the log transformed residuals. The sample path for the test statistic (red) overlayed by 50 approximated sample paths under the null (grey) are displayed. Top panel is the plot for the omnibus test under the different quantiles of covariates. Bottom two panels are the plots for testing the link function (left) and functional form (right)}
\end{figure}

==> code/figure_sim1_mns.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim1_omni_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized omnibus test} \label{fig:sim1_omni_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim1_omni_mns_std.eps} \\
	    \caption{afttestplot: standardized omnibus test} \label{fig:sim1_omni_mns_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim1_link_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized link function test} \label{fig:sim1_link_mns_std} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim1_link_mns_std.eps} \\
	    \caption{afttestplot: standardized link function test} \label{fig:sim1_link_mns_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim1_form_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized functional form test} \label{fig:sim1_form_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim1_form_mns_std.eps} \\
	    \caption{afttestplot: standardized functional form test} \label{fig:sim1_form_mns_std} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:sim1:mns} Plots of sample paths based on the proposed unstandardized and standardized test procedures for Simulation scenario 1 with $\gamma = 0.3$, 20\% censoring rate and the sample size of 300 (non-smoothed). $x$-axis indicates the rank of the log transformed residuals. The sample path for the test statistic (red) overlays by 50 approximated sample paths under the null (grey) are displayed. Top panel is the plot for the omnibus test under the different quantiles of covariates. Bottom two panels are the plots for testing the link function (left) and functional form (right)}
\end{figure}

==> code/figure_sim1_mns_std.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_omni_mns_std.eps} \\
	    \caption{afttestplot: standardized omni function test with \texttt{mns} for model \eqref{model:sim1}} \label{fig:sim1_omni_mns_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_link_mns_std.eps} \\
	    \caption{afttestplot: standardized link function test with \texttt{mns} for model \eqref{model:sim1}} \label{fig:sim1_link_mns_std} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_form_mns_std.eps} \\
	    \caption{afttestplot: standardized form function test with \texttt{mns} for model \eqref{model:sim1}} \label{fig:sim1_form_mns_std} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:sim1:mns:std} Three simple graphs}
\end{figure}

==> code/figure_sim1_mns_unstd.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_omni_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized omni function test with \texttt{mns} for model \eqref{model:sim1}} \label{fig:sim1_omni_mns_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_link_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized link function test with \texttt{mns} for model \eqref{model:sim1}} \label{fig:sim1_link_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim1_form_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test with \texttt{mns} for model \eqref{model:sim1}} \label{fig:sim1_form_mns_unstd} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:sim1:mns:unstd} Three simple graphs}
\end{figure}

==> code/figure_sim2_mis_std.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_omni_mis_std.eps} \\
	   % \caption{afttestplot: standardized omni function test with \texttt{mis} for model \eqref{model:sim2}} \label{fig:sim2_omni_mis_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_link_mis_std.eps} \\
	   % \caption{afttestplot: standardized link function test with \texttt{mis} for model \eqref{model:sim2}} \label{fig:sim2_link_mis_std} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_form_mis_std.eps} \\
	   % \caption{afttestplot: standardized form function test with \texttt{mis} for model \eqref{model:sim2}} \label{fig:sim2_form_mis_std} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:sim2:mis:std} Plots of sample paths based on the proposed standardized test procedures for Simulation scenario 2 with $\gamma = 0.3$, 20\% censoring rate and the sample size of 300. $x$-axis indicates the rank of the log transformed residuals. $x$-axis indicates the rank of the log transformed residuals. The sample path for the test statistic (red) overlays by 50 approximated sample paths under the null (grey) are diplayed. Top panel is the plot for the omnibus test under the different quantiles of covariates. Bottom two panels are the plots for testing the link function (left) and functional form (right)}
\end{figure}

==> code/figure_sim2_mis_unstd.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_omni_mis_unstd.eps} \\
	   % \caption{afttestplot: unstandardized omni function test with \texttt{mis} for model \eqref{model:sim2}} \label{fig:sim2_omni_mis_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_link_mis_unstd.eps} \\
	   % \caption{afttestplot: unstandardized link function test with \texttt{mis} for model \eqref{model:sim2}} \label{fig:sim2_link_mis_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_form_mis_unstd.eps} \\
	   % \caption{afttestplot: unstandardized form function test with \texttt{mis} for model \eqref{model:sim2}} \label{fig:sim2_form_mis_unstd} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:sim2:mis:unstd} Plots of sample paths based on the proposed un-standardized test proposed procedures for Simulation scenario 2 with $\gamma = 0.3$, 20\% censoring rate and the sample size of 300. The sample path for the test statistic (red) overlays by 50 approximated sample paths under the null (grey) are displayed. Top panel is the plot for the omnibus test under the different quantiles of covariates. Bottom two panels are the plots for testing the link function (left) and functional form (right)}
\end{figure}

==> code/figure_sim2_mns.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim2_omni_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized omnibus test} \label{fig:sim2_omni_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim2_omni_mns_std.eps} \\
	    \caption{afttestplot: standardized omnibus test} \label{fig:sim2_omni_mns_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim2_link_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized link function test} \label{fig:sim2_link_mns_std} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim2_link_mns_std.eps} \\
	    \caption{afttestplot: standardized link function test} \label{fig:sim2_link_mns_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim2_form_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized functional form test} \label{fig:sim2_form_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.39]{image/sim2_form_mns_std.eps} \\
	    \caption{afttestplot: standardized functional form test} \label{fig:sim2_form_mns_std} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:sim2:mns} Plots of sample paths based on the proposed unstandardized and standardized test procedures for Simulation scenario 2 with $\gamma = 0.3$, 20\% censoring rate and the sample size of 300 (non-smoothed). $x$-axis indicates the rank of the log transformed residuals. The sample path for the test statistic (red) overlays by 50 approximated sample paths under the null (grey) are displayed. Top panel is the plot for the omnibus test under the different quantiles of covariates. Bottom two panels are the plots for testing the link function (left) and functional form (right)}
\end{figure}

==> code/figure_sim2_mns_std.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_omni_mns_std.eps} \\
	    \caption{afttestplot: standardized omni function test with \texttt{mns} for model \eqref{model:sim2}} \label{fig:sim2_omni_mns_std} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_link_mns_std.eps} \\
	    \caption{afttestplot: standardized link function test with \texttt{mns} for model \eqref{model:sim2}} \label{fig:sim2_link_mns_std} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_form_mns_std.eps} \\
	    \caption{afttestplot: standardized form function test with \texttt{mns} for model \eqref{model:sim2}} \label{fig:sim2_form_mns_std} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:sim2:mns:std} Three simple graphs}
\end{figure}

==> code/figure_sim2_mns_unstd.tex <==
\begin{figure}[htp]
    \centering
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_omni_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized omni function test with \texttt{mns} for model \eqref{model:sim2}} \label{fig:sim2_omni_mns_unstd} \vspace{0em}
    \end{subfigure}
    \\
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_link_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized link function test with \texttt{mns} for model \eqref{model:sim2}} \label{fig:sim2_link_mns_unstd} \vspace{0em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[htp]{0.9\textwidth}
        \centering
        \captionsetup{justification=raggedright,singlelinecheck = false}
	    \includegraphics[scale=0.75]{image/sim2_form_mns_unstd.eps} \\
	    \caption{afttestplot: unstandardized form function test with \texttt{mns} for model \eqref{model:sim2}} \label{fig:sim2_form_mns_unstd} \vspace{0em}
    \end{subfigure}
    \caption{\label{fig:sim2:mns:unstd} Three simple graphs}
\end{figure}

==> code/table_pbc123.tex <==
\begin{table}
    \caption{\label{tab:real:pbc} An omnibus test, link function test, and functional forms of covariates from Model 1, 2, and 3 are shown in Table 3. Both non induced smoothing and induced smoothing methods with a standardized (bold) and unstadardized test statistics are considered.}
    \centering
    \begin{tabular}[t]{ccccccccccccc}
        \toprule
        \multicolumn{1}{c}{ } & \multicolumn{12}{c}{P-value} \\
        \cmidrule(l{3pt}r{3pt}){2-13}
        \multicolumn{1}{c}{ } & \multicolumn{2}{c}{omni} & \multicolumn{2}{c}{link} & \multicolumn{2}{c}{\texttt{bili}} & \multicolumn{2}{c}{\texttt{prot}} & \multicolumn{2}{c}{\texttt{albu}} & \multicolumn{2}{c}{\texttt{age}} \\
        \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} \cmidrule(l{3pt}r{3pt}){10-11} \cmidrule(l{3pt}r{3pt}){12-13}
        model & mns & mis & mns & mis & mns & mis & mns & mis & mns & mis & mns & mis\\
        \midrule
        
        \textbf{} & \textbf{0.020} & \textbf{0.030} & \textbf{0.000} & \textbf{0.010} & \textbf{0.000} & \textbf{0.000} & \textbf{0.725} & \textbf{0.655} & \textbf{0.790} & \textbf{0.800} & \textbf{0.580} & \textbf{0.660}\\

        \multirow{-2}{*}{\hyperlink{model:pbc01}{M1}} & 0.200 & 0.185 & 0.065 & 0.060 & 0.000 & 0.000 & 0.695 & 0.675 & 0.860 & 0.865 & 0.420 & 0.430\\

        \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} \cmidrule(l{3pt}r{3pt}){10-11} \cmidrule(l{3pt}r{3pt}){12-13} 
        
        \textbf{} & \textbf{0.640} & \textbf{0.595} & \textbf{0.165} & \textbf{0.180} & \textbf{0.440} & \textbf{0.400} & \textbf{0.555} & \textbf{0.485} & \textbf{0.800} & \textbf{0.805} & \textbf{0.880} & \textbf{0.820}\\
        
        \multirow{-2}{*}{\hyperlink{model:pbc02}{M2}} & 0.130 & 0.155 & 0.040 & 0.075 & 0.195 & 0.255 & 0.440 & 0.375 & 0.930 & 0.925 & 0.730 & 0.770\\
        
        \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} \cmidrule(l{3pt}r{3pt}){10-11} \cmidrule(l{3pt}r{3pt}){12-13} 
        
        \textbf{} & \textbf{0.650} & \textbf{0.680} & \textbf{0.165} & \textbf{0.205} & \textbf{0.525} & \textbf{0.350} & \textbf{0.505} & \textbf{0.490} & \textbf{0.740} & \textbf{0.770} & \textbf{0.915} & \textbf{0.800}\\
        
        \multirow{-2}{*}{\hyperlink{model:pbc06}{M3}} & 0.225 & 0.215 & 0.110 & 0.110 & 0.275 & 0.290 & 0.405 & 0.430 & 0.900 & 0.880 & 0.710 & 0.710 \\
        \bottomrule
    \end{tabular}
\end{table}

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
